Fast Generating A Large Number of Gumbel-Max Variables

The well-known Gumbel-Max Trick for sampling elements from a categorical distribution (or more generally a nonnegative vector) and its variants have been widely used in areas such as machine learning and information retrieval. To sample a random element $i$ (or a Gumbel-Max variable $i$) in proportion to its positive weight $v_i$, the Gumbel-Max Trick first computes a Gumbel random variable $g_i$ for each positive weight element $i$, and then samples the element $i$ with the largest value of $g_i+\ln v_i$. Recently, applications including similarity estimation and graph embedding require to generate $k$ independent Gumbel-Max variables from high dimensional vectors. However, it is computationally expensive for a large $k$ (e.g., hundreds or even thousands) when using the traditional Gumbel-Max Trick. To solve this problem, we propose a novel algorithm, \emph{FastGM}, that reduces the time complexity from $O(kn^+)$ to $O(k \ln k + n^+)$, where $n^+$ is the number of positive elements in the vector of interest. Instead of computing $k$ independent Gumbel random variables directly, we find that there exists a technique to generate these variables in descending order. Using this technique, our method FastGM computes variables $g_i+\ln v_i$ for all positive elements $i$ in descending order. As a result, FastGM significantly reduces the computation time because we can stop the procedure of Gumbel random variables computing for many elements especially for those with small weights. Experiments on a variety of real-world datasets show that FastGM is orders of magnitude faster than state-of-the-art methods without sacrificing accuracy and incurring additional expenses.

==> preliminary.tex <==
\section{Preliminaries}\label{sec:preliminaries}
{\color{blue}In this section, we first introduce a sketching algorithm $\mathcal{P}$-MinHash \cite{moulton2018maximally} for probability Jaccard similarity estimation as well as a state-of-the-art graph embedding method NodeSketch \cite{yang2019nodesketch}. Then, we demonstrate that the relationships between the two algorithms and the consistent Gumbel-Max variables.

\subsection{Probability Jaccard similarity estimation}
\textbf{Weighted Sampling Property.} $s_1(\vec{v}), \ldots, s_k(\vec{v})$ can be viewed as elements independently sampled from vector $\vec{v}$ with replacement,
where the $i$-th element of $\vec{v}$ is sampled with probability $v^*_i$ for each sample $s_j(\vec{v})$.
Formally, we have
\[
P(s_j(\vec{v}) = i) = \frac{v_j}{\sum_{l=1}^n v_l} = v_i^*,  \quad j = 1,\ldots, k, \quad i = 1, \ldots, n.
\]
The above property enables us to recovery vector $\vec{v}^*$ from $\vec{s}(\vec{v})$ as
\[
\hat v_i^* = \frac{\sum_{j=1}^k s_j(\vec{v})}{k},  \quad i = 1, \ldots, k.
\]
We easily find that 
\[
\mathbb{E}(\hat v_i^*) = v_i^*, \quad \text{Var}(\hat v_i^*) = \frac{v_i^*(1-v_i^*)}{k}.
\]

\textbf{Locality Similarity Hashing Property.} For any two nonnegative vectors $\vec{u}$ and $\vec{v}$, we have
\[
P(s_j(\vec{u}) = s_j(\vec{v})) = \mathcal{J_P}(\vec{u}, \vec{v}) = \sum_{i\in N^+_{\vec{v}}} \frac{1}{\sum_{l=1}^n \max\left(\frac{u_l}{u_i}, \frac{v_l}{v_i}\right)}.
\]
Probability Jaccard similarity  $\mathcal{J_P}(\vec{u}, \vec{v})$ is an effective similarity metric and
can also be used to approximate
the Jaccard similarity of $\vec{u}$ and $\vec{v}$, which is defined as
\begin{equation}\label{eq:minmax}
\mathcal{J_W}(\vec{u}, \vec{v})  = \frac{\sum_{i=1}^n \min\{u_i, v_i\}}{\sum_{i=1}^n \max\{u_i, v_i\}}.
\end{equation}
When $\mathcal{J_W}(\vec{u}, \vec{v}) = \frac{1-p}{1+p}$, Moulton et al.~\cite{MoultonICDM2018} shows that
\[
\frac{1-p}{1+p}\le \mathcal{J_P}(\vec{u}, \vec{v}) \le 1-p.
\]
Since $s_1(\vec{v}), \ldots, s_k(\vec{v})$ are independent, and $s_1(\vec{u}), \ldots, s_k(\vec{u})$ are also independent with each other,
for any $1\le j\le k$ different integers $j_1, \ldots, j_l\in \{1, \ldots, k\}$, we have the following equation
\[
P(s_{j_1} (\vec{u}) = s_{j_1}(\vec{v})\wedge\ldots \wedge s_{j_l} (\vec{u}) = s_{j_l}(\vec{v})) = \left(\mathcal{J_P}(\vec{u}, \vec{v})\right)^l.
\]
The above LSH property enable us to fast search similar vectors and the performance can also be analyzed following the regular LSH framework.

\subsection{NodeSketch}}





